PilotDB: Database-Agnostic Online Approximate Query Processing with A Priori Error Guarantees (Technical Report)

After decades of research in approximate query processing (AQP), its adoption in the industry remains limited. Existing methods struggle to simultaneously provide user-specified error guarantees, eliminate maintenance overheads, and avoid modifications to database management systems. To address these challenges, we introduce two novel techniques, TAQA and BSAP. TAQA is a two-stage online AQP algorithm that achieves all three properties for arbitrary queries. However, it can be slower than exact queries if we use standard row-level sampling. BSAP resolves this by enabling block-level sampling with statistical guarantees in TAQA. We simple ment TAQA and BSAP in a prototype middleware system, PilotDB, that is compatible with all DBMSs supporting efficient block-level sampling. We evaluate PilotDB on PostgreSQL, SQL Server, and DuckDB over real-world benchmarks, demonstrating up to 126X speedups when running with a 5% guaranteed error.

==> figures/alg_overview.tex <==
\newcommand{\myexecute}{DBMS}
\newcommand{\mystatsengine}{StatsEngine}

\begin{algorithm}[t]
    \DontPrintSemicolon
    \SetKwInOut{Input}{Input}\SetKwInOut{Output}{Output}
    \SetKwComment{SideComment}{\textcolor{blue}{//~}}{}
    \SetKwComment{CommentStyle}{\textit{// }}{}
    \SetKwComment{LineComment}{\textcolor{blue}{\textit{/* }}}{\textcolor{blue}{  */}}
    \SetFuncSty{text}
    \SetKwFunction{FTSQA}{\samplingscheme}
    \SetKwFunction{FBS}{\bstats}
    \SetKwFunction{FPilotDB}{\textsc{PilotDB}}
    \SetKwProg{Fn}{Function}{:}{}
    \caption{High-level Algorithm of \name.}
    \label{alg:top-level}
    % I/O setup
    \Input{Input query $\inQ$, relative error $e$, confidence $p$, and the underlying DBMS}
    \Output{Approximate result $R$}
    % algorithm start
    \Fn{\FBS{$\inQ, R_{pilot}, e, p$}}{
        \If{\textsc{NotApproximatable}($\inQ, R_{pilot}$)}{
            $\Phi \leftarrow \emptyset$\;
        }
        \Else{
            \tcp{\textcolor{blue}{\small{Deriving conditions for sampling rates (\S \ref{sec:block})}}}
            $\Phi \leftarrow \textsc{AnalyzeSampleRate}(\inQ, R_{pilot})$
        }
        \Return{$\Phi$}\;
    }
    
    \Fn{\FTSQA{$Q_{in}, e, p,\textsc{StatsEngine},\textsc{DBMS}$}}{
        \tcc{\textcolor{blue}{\small{Sample planning (\S \ref{subsec:plan})}}}
        $\pilotQ \leftarrow \textsc{PilotRewriter}(\inQ)$\;
        $R_{pilot} \leftarrow \textsc{DBMS}(\pilotQ)$\;
        $\Phi \leftarrow \textsc{StatsEngine}(\inQ, R_{pilot}, e, p)$\;
        \If{$\Phi = \emptyset$}{
            $R\leftarrow$\textsc{DBMS}($Q_{in}$)
        }
        \Else{
            \tcc{\textcolor{blue}{\small{Plan optimization (\S \ref{subsec:optimize})}}}
            $\theta \leftarrow \textsc{SamplePlanOptimizer}(\Phi, Q_{in}, DBMS)$\;
            $\finalQ \leftarrow \textsc{Finalrewriter}(\inQ, \theta)$\;
            $R \leftarrow \textsc{DBMS}(\finalQ)$\;
        }
        \Return{$R$}\;
    }

    \Fn{\FPilotDB{$\inQ, e, p, DBMS$}}{
        $\textsc{StatsEngine} \leftarrow \bstats$\;
        $R \leftarrow \samplingscheme(\inQ, e, p, \textsc{StatsEngine}, \textsc{DBMS})$\;
        \Return{$R$}\;
    }
\end{algorithm}

==> figures/fig_augment_quickr.tex <==
\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figures/quickr_augment.pdf}
    \caption{\bstats augments \textsc{Quickr} to achieve up to 60$\times$ better performance.}
    \label{fig:quickr-aug}
\end{figure}

==> figures/fig_comp_quickr.tex <==
\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figures/quickr.pdf}
    \caption{\name outperforms \textsc{Quickr} across all DBMSs.}
    \label{fig:quickr}
\end{figure}

==> figures/fig_final_rule.tex <==
\begin{figure}
    \footnotesize 
    \begin{center}
    \begin{align}
    (1) & \irule{T \ \text{is an input table} \quad T \ \text{is the largest in} \ \inQ \quad \theta\  \text{is the final sample rate}}{T \rightarrow T \ \textbf{\texttt{TABLESAMPLE SYSTEM}}(\theta)} \notag \\
    (2) & \irule{\theta\ \text{is the final sample rate}}{\sqlsum(col) \rightarrow \sqlsum(col)/\theta} \quad (3) \irule{\theta\  \text{is the final sample rate}}{\sqlcount(col) \rightarrow \sqlcount(col)/\theta} \notag
    \end{align}
    \end{center}
    \caption{Rewriting rules for \finalrewriter}
    \label{fig:rule-final}
    \end{figure}

==> figures/fig_more_syntax_pilot_rule.tex <==
\begin{figure}[!t]
    \footnotesize
    \centering
    \[
      \arraycolsep=1.5pt\def\arraystretch{1.1}
      \begin{array}{rrll}
      
        \emph{Table} &
        \sqltable &
        \grammareq &
        ... \ | \ 
        T \sqlspace \textbf{\texttt{TABLESAMPLE SYSTEM}} (\theta)
        \\[2pt]
  
        \emph{Column} & 
        \col & 
        \grammareq & 
        ... \ | \ \textbf{\texttt{PAGELOC}} (T)
        \\[2pt]

        \emph{Sample Rate} &
        \theta &
        \grammareq &
        \text{a real number from 0 to 1}
    \end{array}
    \]
    \vspace{-15pt}
    \caption{Additional syntax for rewritten queries.}
    \label{fig:more-syntax}
\end{figure}
\begin{figure}[!t]
    \footnotesize 
    \begin{center}
    \begin{align}
    (1) & \irule{T \ \text{is an input table} \quad T \ \text{is the largest in} \ \inQ \quad \theta\  \text{is the pilot sample rate}}{T \rightarrow T \ \textbf{\texttt{TABLESAMPLE SYSTEM}}(\theta)} \notag \\
    (2) & \irule{T \ \text{is an input table} \ \quad T \ \text{is the largest in} \ \inQ}{\gcols \rightarrow \bigl(\gcols, \textbf{\texttt{PAGELOC}}(T)\bigr)} \notag \quad (3)\irule{}{ a_1 \ aop \ a_2  \rightarrow (a_1, a_2) } \notag \\
    (4) & \irule{}{\sqlavg(col) \rightarrow \bigl(\sqlsum(col), \sqlcount(col)\bigr)} \notag
    \end{align}
    \end{center}
    \caption{Rewriting rules for \pilotrewriter}
    \label{fig:rule-pilot}
    \end{figure}

==> figures/fig_pilot_principles.tex <==
\begin{figure}[t!]
    \begin{subfigure}[t]{0.48\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/tail_bounds.pdf}
        \caption{Sub-Gaussian distributions (\eg, normal, $\chi^2$, etc.) have exponentially decreasing tails.}
        \label{fig:tail-bound}
    \end{subfigure}%
    \hfill
    \begin{subfigure}[t]{0.48\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/interval_estimation.pdf}
        \caption{Estimation statistics (\eg, variance) with intervals (\eg, upperbounds).}
        \label{fig:interval-estimation}
    \end{subfigure}
    \caption{Illustrations of tail bounds and interval estimations.}
\end{figure}

==> figures/fig_rules.tex <==
\begin{figure}
  \footnotesize
  \centering
  \[
    \arraycolsep=1.5pt\def\arraystretch{1.1}
    \begin{array}{rrll}
    
      \emph{Table} &
      \sqltable &
      \grammareq &
      ... \ | \ 
      T \sqlspace \textbf{\texttt{TABLESAMPLE SYSTEM}} (\theta)
      \\[2pt]

      \emph{Column} & 
      \col & 
      \grammareq & 
      ... \ | \ \textbf{\texttt{PAGELOC}} (T)
      \\[2pt]
  \end{array}
  \]
  \vspace{-15pt}
  \caption{Additional syntax for rewritten queries.}
  \label{fig:more-syntax}
\end{figure}

\begin{figure}
    \footnotesize 
    \begin{center}
    \begin{align}
    (1) & \irule{T \ \text{is an input table} \quad T \ \text{is largest in} \ \inQ \quad \theta\  \text{is the pilot sample rate}}{T \ \textbf{\texttt{TABLESAMPLE}}(\theta) \in \pilotQ} \notag \\
    (2) & \irule{T \ \text{is an input table} \ \quad T \ \text{is largest in} \ \inQ}{\textbf{\texttt{PAGELOC}}(T) \in \texttt{GroupingCols}(\pilotQ)} \notag  \\
    (3) & \irule{(t_1 \ aop \ t_2 ) \in \inQ}{[t_1, t_2] \in  \pilotQ} \notag \quad (4) \irule{\sqlavg(col) \in \inQ}{[\sqlsum(col), \sqlcount(col)] \in \pilotQ}
    \end{align}
    \end{center}
    \caption{Inference rules for \pilotrewriter}
    \label{fig:rule-pilot}
    \end{figure}
    
\begin{figure}
  \footnotesize 
  \begin{center}
  \begin{align}
  (1) & \irule{T \ \text{is an input table} \quad T \ \text{is largest in} \ \inQ \quad \theta\  \text{is the final sample rate}}{T \ \textbf{\texttt{TABLESAMPLE}}(\theta) \in \finalQ} \notag \\
  (2) & \irule{\sqlsum(col) \in \inQ \quad \theta\  \text{is the sample rate}}{\sqlsum(col)/\theta \in  \finalQ} \notag \\
  (3) &  \irule{\sqlcount(col) \in \inQ \quad \theta\  \text{is the sample rate}}{\sqlcount(col)/\theta \in  \finalQ} \notag
  \end{align}
  \end{center}
  \caption{Inference rules for \finalrewriter}
  \label{fig:rule-final}
  \end{figure}

==> figures/fig_syntax.tex <==

\begin{figure}[!t]
    \footnotesize
    \centering
    \[
    \arraycolsep=1.5pt\def\arraystretch{1.1}
    \begin{array}{rrll}

    \emph{Expression} & 
    \sqlexpr & 
    \grammareq & 
    \emph{const} \ | \ \col \ | \ T \ | \ Q
    \\[2pt] 
    
    \emph{Query} & 
    \query & 
    \grammareq & 
    \sqlselect \sqlspace \targetlist \sqlspace \sqlfrom \sqlspace \sqltable \sqlspace \sqlwhere \sqlspace \sqlpredicate \\ 
    & & \ \ \ | &  
    \sqlselect \sqlspace \targetlist \sqlspace \sqlfrom \sqlspace \sqltable \sqlspace \sqlgroupby \sqlspace \gcols \sqlspace \sqlhaving \sqlspace \sqlpredicate \\ 
    & & \ \ \ | &  
    \sqlselect \sqlspace \targetlist \sqlspace \sqlfrom \sqlspace \sqltable \sqlspace \sqlgroupby \sqlspace \gcols \sqlspace \sqlhaving \sqlspace \sqlpredicate \sqlspace \sqlorderby \sqlspace \targetlist  \\ 
    & & \ \ \ | &  
    \makecell[l]{\sqlselect \sqlspace \targetlist \sqlspace \sqlfrom \sqlspace \sqltable \sqlspace \sqlgroupby \sqlspace \gcols \sqlspace \sqlhaving \sqlspace \sqlpredicate \sqlspace \sqlorderby \sqlspace \targetlist \\ \sqlspace\sqlspace \sqllimit \sqlspace \emph{a positive integer}}
    \\[2pt]

    \emph{Table} &
    \sqltable &
    \grammareq &
    \emph{an input table}\\
    & & \ \ \ | &  
    \sqlselect \sqlspace \cols \sqlspace \sqlfrom \sqlspace \sqltable \sqlspace \sqlwhere \sqlspace \sqlpredicate \\
    & & \ \ \ | &  
    \sqltable \sqlspace \sqlinnerjoin \sqlspace \sqltable \sqlspace \sqlon \sqlspace \sqlpredicate 
    \ | \ \sqltable \sqlspace \textbf{\texttt{CROSS JOIN}} \sqlspace \sqltable \sqlspace \sqlon \sqlspace \sqlpredicate \\
    & & \ \ \ | &  
    \sqltable \sqlspace \sqlleftjoin \sqlspace \sqltable \sqlspace \sqlon \sqlspace \sqlpredicate
    \ | \ \sqltable \sqlspace \textbf{\texttt{RIGHT JOIN}} \sqlspace \sqltable \sqlspace \sqlon \sqlspace \sqlpredicate \\
    & & \ \ \ | &  
    \sqltable \sqlspace \sqlunionall \sqlspace \sqltable \sqlspace
    \\[2pt]

    \emph{Target List} & 
    \targetlist & 
    \grammareq & 
    % [ \target \sqlspace \sqlas \sqlspace \colalias, \mydots, \target \sqlspace \sqlas \sqlspace \colalias ]
    (t, \mydots, t)
    % \\
    % & & \ \ \ | &  
    % \sqldistinct \sqlspace [ \target \sqlspace \sqlas \sqlspace \colalias, \mydots, \target \sqlspace \sqlas \sqlspace \colalias ] 
    %\rui{add DISTINCT?}
    \\[2pt]

    \emph{Target} & 
    \target & 
    \grammareq & 
    \col \ | \ \col \ \emph{aop}\ \col \ | \ \col \ \emph{aop} \ \emph{const} \ | \ \aggregate
    \\[2pt]
    
    \emph{Aggregate} & 
    \aggregate & 
    \grammareq & 
    \agg(\col) \ | \ \aggregate \ \emph{aop} \ \aggregate \ | \ \emph{const} \ \emph{aop} \ \aggregate
    \\[2pt]

    \emph{Group Col.} & 
    \gcols & 
    \grammareq & 
    (\col, \mydots, \col)
    \\[2pt]
    
    \emph{Column} & 
    \col & 
    \grammareq & 
    \emph{a column from an input table} 
    \\[2pt]

    \emph{Agg. Func.} & 
    \agg & 
    \grammareq & 
    \sqlavg \ | \ \sqlsum \ | \ \sqlcount 
    \\[2pt] 
    
    \emph{Condition} & 
    \sqlpredicate & 
    \grammareq & 
    \sqlexpr \sqlspace \emph{op} \sqlspace \sqlexpr 
    \ | \ \textbf{\texttt{EXISTS}} \sqlspace \sqlexpr 
    \ | \ \aggregate \sqlspace \emph{cop} \sqlspace \sqlexpr
    \ | \ \aggregate \sqlspace \emph{cop} \sqlspace \aggregate \\ 
    & & \ \ \ | &
    \sqlpredicate \sqlspace \texttt{\textbf{AND}} \sqlspace \sqlpredicate \ | \ \sqlpredicate \sqlspace \texttt{\textbf{OR}} \sqlspace \sqlpredicate \ | \ \texttt{\textbf{NOT}} \sqlspace \sqlpredicate
    \\[2pt] 

    \emph{Operator} & 
    \emph{op} &
    \grammareq &
    <> \ | \ = \ | \ \emph{cop}
    \\[2pt]

    \emph{Comp. Op.} & 
    \emph{cop} &
    \grammareq &
    > \ | \ < \ | \ >= \ | \ <= \ | \ \textbf{\texttt{IN}} \ | \ \textbf{\texttt{NOT IN}}
    \\[2pt]

    \emph{Arith. Op.} & 
    \emph{aop} &
    \grammareq &
    + \ | \ * \ | \ \backslash
    \\[2pt]
    
    \end{array}
    \]
    \vspace{-15pt}
    \caption{Syntax of supported queries.}
    \label{fig:syntax}
    % \vspace{-20pt}
    \end{figure}
    
    
    

==> figures/fig_tablesample.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=0.4\linewidth]{figures/tablesample.pdf}
    \caption{Micro experiment}
    \label{fig:archi}
\end{figure}

==> figures/tab_block_estimations.tex <==
\begin{table*}[t]
    \small
    \begin{minipage}{0.63\linewidth}
        \centering
        \caption{Transformation of common aggregates from row-oriented estimators to page-oriented estimators equivalently.}
        \label{tab:page-agg}
        \begin{tabular}{c|cc|cc}
            \toprule
            \multirow{2}{*}{Aggregate} & \multicolumn{2}{c|}{Exact value} & \multicolumn{2}{c}{Estimator} \\ \cline{2-5}
                    & Row & Page & Row & Page \\
            \midrule
            \acount  & $\sum_{i=1}^N Q_i$       & $N \cdot  \mu_Q$ & $\left(\sum_{i=1}^n Q_i\right) \big / \theta$ & $(n / \theta) \cdot \bar Q$\\
            \asum    & $\sum_{i=1}^N \sum_{j=1}^{Q_i} X_{i,j}$& $N \cdot  \mu_S$ & $\left(\sum_{i=1}^n \sum_{j=1}^{Q_i} X_{i,j}\right) \big/ \theta$ & $(n / \theta) \cdot \bar S$\\
            \aavg    & $\mu_X$ & $\mu_S / \mu_Q$ & $\left(\sum_{i=1}^n \sum_{j=1}^{Q_i} X_{i,j}\right) \big/ \left(\sum_{i=1}^N Q_i\right)$ & $\bar S / \bar Q$ \\
            \bottomrule
        \end{tabular}
    \end{minipage}%
    \hfill
    \begin{minipage}{0.34\linewidth}
        \centering
        \caption{Summary of upper bounds of relative errors of composite estimators with multiplication, division, and addition.}
        \label{tab:error-prop}
        \begin{tabular}{cc}
        \toprule
        \makecell[c]{Composite\\estimator} & Upper bound of relative error \\
        \midrule
        $\hat x \cdot \hat y$ & $e_x + e_y + e_x \cdot e_y$ \\
        $\hat x / \hat y$ & $(e_x+e_y)/(1+\min(e_x, e_y))$ \\
        $\hat x + \hat y$ & $\max(e_x, e_y)$\\
        \bottomrule
        \end{tabular}
    \end{minipage}
    
\end{table*}

==> figures/tab_notation.tex <==
\begin{table}
    \centering
    \caption{Notations}
    \label{tab:notation}
    \begin{tabular}{cl}
        \toprule
        Symbol & Meaning \\
        \midrule
        $p$ & user-specified overall failure probability \\
        $e$ & user-specified maximum relative error \\
        $g$ & user-specified minimum group size \\
        $G, G'$ & groups of the exact or approximate query \\
        $G_i$ & $i$-th group \\
        $A_{i,j}, \hat A_{i,j}$ & (estimated) aggregate of group $G_i$ and column $j$ \\
        $p^{(g)}$ & probability of missing a group of size $> g$ \\
        $p^{(e)}_{i,j}$ & probability of $\hat A_{i,j}$ having relative error $> e$ \\
        $R$ & table \\
        $f$ & aggregate function \\
        $\mathcal{B}$ & block sampling \\
        \bottomrule
    \end{tabular}
\end{table}

==> figures/tab_perf.tex <==
\begin{table}
    \centering
    \caption{\name accelerates over 80\% of queries and achieves speedups by up to two orders of magnitude.}
    \label{tab:perf}
        % \small
        \begin{tabular}{cccc}
            \toprule
            & PostgreSQL & SQL Server & DuckDB \\
            \midrule
        Query coverage & 80.0\% & 82.9\% & 82.9\% \\
        G.M. speedup   & 5.90$\times$ & 5.63$\times$ & 1.84$\times$ \\
        Max. speedup   & 126$\times$  & 56.5$\times$ & 13.2$\times$ \\
        \bottomrule
        \end{tabular}
\end{table}

==> tex/detailed_related_work.tex <==
In this section, we review the related work on online AQP, offline AQP, and 
online aggregation (OLA). 

\minihead{Online AQP} 
Generating and analyzing samples of large tables upon query arrival is widely 
studied in prior AQP systems and algorithms \cite{simple-random-sampling,
group-by-sample,sampling-algebra,analytical-bootstrap,abs,quickr,idea}. Prior 
work has considered random sampling as a standard operation in query processing 
to estimate aggregates and used analytical confidence intervals to measure the 
error of estimations \cite{simple-random-sampling,group-by-sample,sampling-algebra}. 
Bootstrap techniques have been explored as an alternative method for constructing 
confidence intervals in AQP, involving the creation of multiple resamples from 
an initial sample \cite{bootstrap,analytical-bootstrap,abs}. However, since 
bootstrap is simulation-based, it cannot be applied to provide a priori error 
guarantees. As a step further to accelerate complex queries, \textsc{Quickr} 
injects sampling operations in the query plan level and integrate sample planning
with query optimization to achieve query acceleration and a priori error guarantees 
\cite{quickr}. Additionally, \textsc{Idea} reuses previous query results to 
accelerate future approximate queries \cite{idea}. More recently, \textsc{Taster} 
combines online and offline methods by caching the online samples and reusing 
them for future queries to achieve faster execution \cite{taster}.

Although existing online AQP systems can provide reliable answers by measuring 
post-hoc errors, they cannot provide a priori error guarantees without modifying
the underlying DBMS. Recent advances develop sampling injection and optimization 
algorithms. This requires significant modifications to the query optimization 
and execution engine of existing DBMSs. Despite these modifications, state-of-the-art 
methods still slow down a part of queries compared with exact execution 
\cite{quickr,taster} or lead to errors as big as 100\% \cite{quickr}.

\minihead{Offline AQP} 
Prior work developed two types of offline AQP methods. First, previous work 
investigates summary-based methods, such as sketches \cite{sketch-tutorial,
bias-aware-sketch,count-filter-sketch}, histograms \cite{count-est,
histogram-selectivity,digithist}, and wavelets \cite{wavelet,distributed-wavelet}.
Their primary idea is compressing or summarizing columns through numeric 
transformations. Therefore, they cannot process queries with non-numeric columns, 
such as categorical columns, or with complex relational operations, such as join 
and grouping.

Second, prior work developed the method of generating offline samples to answer 
online queries \cite{join-synopses,aqua-sigmod,aqua,icicles,congressional-sample,
start,outlier,sample-selection,blinkdb,sample+seek,verdictdb,baq,taster}. Aqua 
first developed the method of rewriting queries with pre-computed samples to 
answer approximate queries \cite{join-synopses,congressional-sample,aqua-sigmod,
aqua}. Subsequently, various optimizations in offline sample creation have been 
proposed, such as weighted sampling \cite{icicles,sample-selection}, stratified 
sampling \cite{start}, and outlier index \cite{outlier}. Prior work has explored 
guaranteeing errors a priori by generating specialized samples for non-nested 
queries \cite{baq}, sparse data distribution \cite{error-bounded-stratified}, 
queries over specific columns \cite{blinkdb}, and queries with specific 
selectivities \cite{sample+seek}. Furthermore, \textsc{VerdictDB} proposed 
developing offline AQP as a middleware to avoid modifications to DBMSs 
\cite{verdictdb}. 

Offline sampling-based AQP methods have two fundamental limitations. First, their 
a priori error guarantees are inherently limited to predictable workloads 
\cite{blinkdb,sample+seek,error-bounded-stratified,baq}. For example, \textsc{BlinkDB} 
requires that incoming queries output columns in a pre-defined column set; 
\textsc{Sample+Seek} relies on the pre-knowledge of the query selectivity to 
select the right processing policy (\ie, sample or seek); \textsc{Baq} only 
supports non-nested queries. Moreover, maintaining offline samples requires 
special effort and costs, including regularly refreshing samples to ensure 
statistical correctness and regenerating samples when the database changes 
\cite{aqua,blinkdb,verdictdb}. Nevertheless, offline sampling methods can be 
applied to complement \name to achieve a more comprehensive query acceleration.

\minihead{Online Aggregation} 
Previous research has explored interactive processing of aggregation queries, 
providing initial results immediately and improving accuracy as more data is 
sampled \cite{online-aggregation,ripple-join,dbo,turbo-dbo,cosmos,gola,deepola,
progressivedb}. OLA, first proposed by Hellerstein et al. 
\cite{online-aggregation}, has been subsequently improved to support join 
queries \cite{ripple-join,wander-join}, scalable processing on large databases 
\cite{dbo,turbo-dbo}, processing multiple queries simultaneously \cite{cosmos}, 
and complex aggregates \cite{gola}. Furthermore, \textsc{ProgressiveDB} explored 
online aggregation as an extension to existing DBMSs using progressive views 
\cite{progressivedb}. More recently, \textsc{DeepOLA} tackled nested queries for 
online aggregation \cite{deepola}. 

Although OLA techniques can continuously update confidence intervals, it is 
invalid to consider the monitored confidence interval as an error guarantee due 
to the problem of peeking at early results \cite{peeking}. Nevertheless, OLA can 
be integrated with the second stage of \name to provide constantly updating 
results, thereby improving the interactivity and user experience.

==> tex/determining_large_tables.tex <==
Given $k$ tables in the query, \name determines which table(s) to sample 
when executing pilot query and final query. The pilot query only samples the 
table that is most expensive to load. \name estimates the cost of table loading
in two steps. First, \name checks how the underlying DBMS will load the table by
obtaining a query plan from the DBMS without executing the query.
\begin{enumerate}[leftmargin=*]
    \item If DBMS seeks the table, PilotDB will avoid sampling on 
    it because seeking is faster than sampling. This often happens when 
    there are indices on that table and the selectivity of the predicate is 
    small.
    \item If DBMS scans the table, PilotDB will consider it as a 
    candidate to execute sampling. This is because scanning on fact tables 
    is much more expensive than sampling even with predicates.
\end{enumerate}
Second, \name queries estimated table cardinality maintained by the
DBMS. Both steps can be efficiently completed within 10ms. Finally, the pilot 
query samples the candidate table determined in the first step with the greatest 
estimated cardinality.

The sampling plan optimization also follows the same steps to determine
the tables to search the optimal sampling plan on. To reduce the 
optimization complexity, we constrain the tables to the set of candidate tables
obtained in the first step and tables with estimated cardinality greater than
1 million rows.

\minihead{Case Study 1} To process the following 
query from TPC-DS on SQL Server, \name first issues \texttt{SET SHOWPLAN\_XML 
ON;} and the query to get the query plan. Then, \name finds 
\texttt{@PhysicalOp=Clustered Index Seek} on the table \texttt{lineitem} in the 
query plan, indicating that SQL Server seeks \texttt{lineitem}. Since other 
tables are small, \name decides not to execute sampling on this query.
\begin{lstlisting}[keywords={SELECT,SUM,FROM,TABLESAMPLE,WHERE,DATE,AND,SYSTEM,JOIN,ON,GROUP,BY,ORDER,LIMIT}]
SELECT dt.d_year, item.i_brand_id brand_id, 
    item.i_brand brand,
    SUM(ss_sales_price) sum_agg
FROM date_dim dt, store_sales, item
WHERE dt.d_date_sk = store_sales.ss_sold_date_sk
  AND store_sales.ss_item_sk = item.i_item_sk
  AND item.i_manufact_id = 816 AND dt.d_moy = 11
GROUP BY dt.d_year, item.i_brand, item.i_brand_id
ORDER BY dt.d_year, sum_agg DESC, brand_id
LIMIT 100;
\end{lstlisting}

\minihead{Case Study 2} To process the following 
query from TPC-H on PostgreSQL, \name first issues \texttt{EXPLAIN {query};} 
to get the query plan. Then, \name finds \texttt{Seq Scan on lineitem} and 
\texttt{Seq Scan on part} in the query plan, indicating that PostgreSQL scans 
both \texttt{lineitem} and \texttt{part}. Thus, \name searches for sample plans 
that sample \texttt{lineitem}, \texttt{part}, or both.

\begin{lstlisting}[keywords={SELECT,SUM,FROM,THEN,END,AS,ELSE,WHERE,DATE,AND,SYSTEM,JOIN,ON,GROUP,BY,ORDER,LIMIT}]
SELECT 100.00 * SUM(case when p_type like 'PROMO%' 
        THEN l_extendedprice * (1 - l_discount)
        ELSE 0 END) / 
    SUM(l_extendedprice * (1-l_discount)) AS promo_revenue
FROM lineitem, part
WHERE l_partkey = p_partkey 
    AND l_shipdate >= DATE '1995-09-01'
    AND l_shipdate < DATE '1995-09-01' + '1' month;
\end{lstlisting}


==> tex/prelim.tex <==
\section{Preliminaries}

\begin{lemma}\label{lemma:iid-sample-1}
Let $X_1, \ldots, X_n$ be a sequence of i.i.d. random variables with the expected value $\mu$ and finite variance $\sigma^2$. Suppose $\bar X$ is the sample mean (Eq. \ref{eq:sample-mean}) and $\hat\sigma^2$ is the unbiased sample variance (Eq. \ref{eq:sample-var}).
\begin{align}
\bar X &= \frac{\sum_{i=1}^n X_i}{n} \label{eq:sample-mean} \\
\hat\sigma^2 &= \frac{\sum_{i=1}^n \left(X_i - \bar X\right)}{n-1} \label{eq:sample-var} 
\end{align}

We have the following confidence intervals for $\mu$ and $\sigma$.
\begin{align}
\lim_{n\rightarrow \infty} \mathbb{P}\left[L^{(t)}_{\mu}(\bar X, \hat \sigma, n, \delta/2) \le \mu \le U^{(t)}_{\mu}(\bar X, \hat \sigma, n, \delta/2) \right] & = 1-\delta \notag \\
\lim_{n\rightarrow \infty} \mathbb{P}\left[L_{\sigma}(\hat \sigma, n, \delta/2) \le \sigma \le U_{\sigma}(\hat \sigma, n, \delta/2) \right] & = 1-\delta \notag
\end{align}
where
\begin{gather}
L^{(t)}_{\mu}(\bar X, \hat \sigma, n, \delta) = \bar X - t_{n-1,1-\delta} \frac{\hat \sigma}{\sqrt{n}}, \\
U^{(t)}_{\mu}(\bar X, \hat \sigma, n, \delta) = \bar X + t_{n-1,1-\delta} \frac{\hat \sigma}{\sqrt{n}} \label{eq:mean-bounds-t}\\
L_{\sigma}(\hat \sigma, n, \delta) = \sqrt{\frac{n-1}{\chi^2_{n-1, 1-\delta}}} \hat\sigma,  \quad
U_{\sigma}(\hat \sigma, n, \delta) = \sqrt{\frac{n-1}{\chi^2_{n-1, \delta}}} \hat\sigma \label{eq:std-bounds}
\end{gather}
$t_{n-1,1-\delta}$ is the upper $\delta$ critical point of Student's t distribution with $n-1$ degrees of freedom. 
$\chi^2_{n-1, \delta}$ is the lower $\delta$ critical point of chi-squared distribution with $n-1$ degrees of freedom.

If we know the variance $\sigma^2$, we can have the following confidence interval for $\mu$.
\begin{equation}
\lim_{n \rightarrow \infty}\mathbb{P}\left[L^{(z)}_\mu (\bar X, \sigma, n, \delta/2) \le \mu \le U^{(z)}_\mu (\bar X, \sigma, n, \delta/2)\right] = 1- \delta \notag
\end{equation}
where
\begin{gather}
L^{(z)}_{\mu}(\bar X, \sigma, n, \delta) = \bar X - z_{1-\delta} \frac{\sigma}{\sqrt{n}}, \\
U^{(z)}_{\mu}(\bar X, \sigma, n, \delta) = \bar X + z_{1-\delta} \frac{\sigma}{\sqrt{n}}, \label{eq:mean-bounds-z}
\end{gather}
$z_{1-\delta}$ is the upper $\delta$ critical point of standard normal distribution.
\end{lemma}

\begin{lemma}\label{lemma:binomial}
Suppose we have a sequence of $N$ independent experiments. Each experiment is either successful or not successful with a fixed success probability $\theta$. We have the following confidence interval for the number of successes $n$.
\begin{equation}
    \lim_{N \rightarrow \infty} \mathbb{P}\left[L_n(N, \theta, \delta/2) \le n \le U_n(N, \theta, \delta/2)\right] = 1- \delta \label{eq:bernoulli-n-bounds}
\end{equation}
where 
\begin{gather}
    L_n(N, \theta, \delta) = N\theta - z_{1-\delta}\sqrt{N\theta(1-\theta)} \\
    U_n(N, \theta, \delta) = N\theta + z_{1-\delta}\sqrt{N\theta(1-\theta)}
\end{gather}
$z_{1-\delta/2}$ is the upper $\delta/2$ critical point of standard normal distribution.
\end{lemma}
